Reducing Seed Bias in Respondent-Driven Sampling by Estimating Block Transition Probabilities

Respondent-driven sampling (RDS) is a popular approach to study marginalized or hard-to-reach populations. It collects samples from a networked population by incentivizing participants to refer their friends into the study. One major challenge in analyzing RDS samples is seed bias. Seed bias refers to the fact that when the social network is divided into multiple communities (or blocks), the RDS sample might not provide a balanced representation of the different communities in the population, and such unbalance is correlated with the initial participant (or the seed). In this case, the distributions of estimators are typically non-trivial mixtures, which are determined (1) by the seed and (2) by how the referrals transition from one block to another. This paper shows that (1) block-transition probabilities are easy to estimate with high accuracy, and (2) we can use these estimated block-transition probabilities to estimate the stationary distribution over blocks and thus, an estimate of the block proportions. This stationary distribution on blocks has previously been used in the RDS literature to evaluate whether the sampling process has appeared to `mix'. We use these estimated block proportions in a simple post-stratified (PS) estimator that greatly diminishes seed bias. By aggregating over the blocks/strata in this way, we prove that the PS estimator is $\sqrt{n}$-consistent under a Markov model, even when other estimators are not. Simulations show that the PS estimator has smaller Root Mean Square Error (RMSE) compared to the state-of-the-art estimators.

==> diagram1.tex <==
\begin{wrapfigure}[5]{r}{0.3\textwidth}
	\usetikzlibrary{matrix}
	\def\leftbracket{[}
	\def\rightbracket{]}
	
	\tikzset{my arrow/.style={
			blue!60!black,
			-latex
		}
	}
\begin{tikzpicture}
\matrix[matrix of math nodes, row sep=4mm] (M) {
 & \hat{C}_{0,1} & \hat{C}_{0,2} & ... & \hat{C}_{0,\tilde{n}_0} &  \\
 & \hat{C}_{1,1} & \hat{C}_{1,2} & ... & \hat{C}_{1,\tilde{n}_1} &  \\
 &\vdots             & \vdots        & \vdots & \vdots&\\
 & \hat{C}_{N-1,1} & \hat{C}_{N-1,2} & ... & \hat{C}_{N-1,\tilde{n}_{N-1}} &\\
};

\draw[my arrow] (M-1-2) to (M-1-5);
\draw[my arrow] (M-1-5) to (M-2-2);
\draw[my arrow] (M-2-2) to (M-2-5);
\draw[my arrow] (M-2-5) to (M-3-2);
\draw[my arrow] (M-3-2) to (M-3-5);
\draw[my arrow] (M-3-5) to (M-4-2);
\draw[my arrow] (M-4-2) to (M-4-5);
\end{tikzpicture}
\end{wrapfigure}

==> gmm.tex <==
\section{``Given" Markov Model}\label{sec: gmm}

\snote{S: This whole section uses a different model, which is confusing. It is more motivation than anything. It should be moved to the motivation section and the distinction with our true model should be made clear.}

The RDS sample recruiting process can be represented by a Hidden Markov Model (\cite{krogh1994hidden}), with $\{Z_{\tau}\}_{\tau\in\mathbbm{T}}$ as the hidden states and $\{Y_{\tau}\}_{\tau\in\mathbbm{T}}$ as the outcomes.  In this paper, we assume we observe the block variables $\{Z_{\tau}\}$, so we call the model a ``Given" Markov Model instead \snote{S: I don't think that's a good name. It's just a Markov model. And the hidden Markov model analogy is misleading -- it's not linear.}.

Denote $\mathcal{D}(\tau)\in\mathbbm{T}$ as the set of sample $\tau$ and all its descendants in $\mathbbm{T}$.  Denote $S$ as the set of all the possible values for the variable of interest, e.g. $S = \{0,1\}$ for the indicator of HIV status.  In the ``Given" Markov Model, we still have the properties of the Hidden Markov Models,
$$\mathbbm{P}(Z_{\tau} = k \ |\  Z_{\tau'}, Z_{\sigma}: \sigma\in\mathcal{D}(\sigma)^c\}) = \mathbbm{P}(Z_{\tau} = u \ |\ Z_{\tau'}), \text{ for all $k\in\{1,\dots, K\}$},$$
$$\text{and } \mathbbm{P}(Y_{\tau} = s\ |\ Z_{\tau}: \tau\in\mathbbm{T}) = \mathbbm{P}(Y_{\tau} = s\ |\ Z_{\tau})\text{ for all $s\in S$},$$
\snote{S: I'm not following. $Y_\tau$ is a function of the node -- not the block. And you cannot pretend like the transition between blocks does not depend on the node. This is a different model than what was introduced earlier in the paper.}
but we assume the states, $\{Z_{\tau}\}_{\tau\in\mathbbm{T}}$, are visible.

For each block $k$ and each possible value for $y(i)$'s, $s\in S$, we define $q_k(s) = \mathbbm{P}(y(i) = s \ |\ z(i) = k)$ as the probability for a node in the block taking value $s$ \snote{S: Same.}, and $n_k(s) = \sum\limits_{\tau\in\mathbbm{T}_k}\ind\{Y_{\tau} = s\}$ as the number of samples in block $k$ taking value $s$. 

\begin{lemma}\label{lem: gmm}
	Under the ``Given" Markov Model, the MLE of $P^{(B)}$ is $\hat{Q}_R$, and $\hat{\pi}_k^{(B)}$ is the plug-in MLE of $\pi_k$ for each block $k\in \{1,\dots, K\}$.
\end{lemma}

\begin{proof}
	Recall for each block $k\in\{1,\dots, K\}$ and possible value for outcome $s\in S$, $n_k =  |\mathbbm{T}_k|$ and $n_k(s) = \sum\limits_{\tau\in\mathbbm{T}_k}\ind\{Y_{\tau} = s\}$.  For any block $k$, we define the number of referrals from block $k$ as
	\begin{equation}\label{def: n_k'}
	n_{k'} = \sum\limits_{\tau\in\mathbbm{T}}\ind\{Z_{\tau'} = k\}.
	\end{equation} 
	For any two blocks $u,v\in\{1,\dots, K\}$, we define the number of referrals between block $u$ and block $v$ as 
	\begin{equation}\label{def: n_u'v}
	n_{u'v} = \sum\limits_{\tau\in\mathbbm{T}}\ind\{Z_{\tau'} = u, Z_{\tau} = v\}.  
	\end{equation}
	Note that $\hat{Q}_{uv} = n_{u'v}/n$ and $[\hat{Q}_R]_{uv} = n_{u'v}/n_{u'}$. \snote{S: $\hat{Q}_R$ is not technically the same as what we had before because it's actually a different model. I find this confusing.}
	
	Under the ``Given" Markov Model, the likelihood  is $$\Pi_{i = 1}^n [P^{(B)}]_{z_{i'}z_i} q_{z_i}(y_i) 
	= \{\Pi_{u,v = 1}^K [P^{(B)}]_{u'v}^{n_{u'v}}\}\cdotp \{\Pi_{k = 1}^K\Pi_{s} q_k(s)^{n_k(s)}\}.$$ 
    \snote{S: Again, this is not the model introduced in the paper. The $y$ variables are not a function of the block only.}
	
	A straightforward calculation leads to the fact that the MLE $\hat{P}^{(B)}$ has elements
	$$[\hat{P}^{(B)}]_{uv} = n_{u'v}/n_{u'} = [\hat{Q}_R]_{uv}, \quad \text{ for all } u,v\in\{1,\dots, K\}.$$
	
	Recall the $\hat{\bfpi}^{(B)} = (\hat{\pi}_k^{(B)})_k$ is the stationary distribution of $\hat{Q}_R$.  Thus under the ``Given" Markov Model, for each block $k\in \{1,\dots, K\}$, $\hat{\pi}_k^{(B)}$ is the plug-in MLE of $\pi_k$.  Together with $\hat{\mu}_{k\text{VH}}$'s and $H^{(\delta_k)}$'s,  they consist of the PS estimator defined in \eqref{eq: s-vh}.
	
\end{proof}
